Story-thinking, computational-thinking, programming and software engineering

Working with stories and working with computations require very different modes of thought. We call the first mode "story-thinking" and the second "computational-thinking". The aim of this curiosity-driven paper is to explore the nature of these two modes of thinking, and to do so in relation to programming, including software engineering as programming-in-the-large. We suggest that story-thinking and computational-thinking may be understood as two ways of attending to the world, and that each both contributes and neglects the world, though in different ways and for different ends. We formulate two fundamental problems, i.e., the problem of "neglectful representations" and the problem of oppositional ways of thinking. We briefly suggest two ways in which these problems might be tackled and identify candidate hypotheses about the current state of the world, one assertion about a possible future state, and several research questions for future research.

==> archive.tex <==

\section*{Notes and other detritus}
\subsection{Problems}

Fletcher: the problem of unscrewing a nut.

\subsection{Fiction}

One aspect of stories that may be uncomfortable to some programmers, and perhaps also some researchers, is the sense that a story, by its nature, is often false or untrue. The six-word story itself is not actually true, though one can imagine many real-world occurrences. The six-word story represents as true the content of the story, even though the story itself is not true. It can be helpful to distinguish between the truth \textit{within} the story and the meaning \textit{of} the story. A factually untrue story can convey a great deal of genuine meaning.

Programmers, and more generally software engineers, deal with fictions as part of their professional roles. A user story is an artifice and therefore a fiction. A class diagram, as part of a software design for a future software system, is a fiction, for the software does not yet exist. Computer science, and then artificial intelligence, has reasoned with two fictions, Turing's \textit{Imitation Game} and Searle's \textit{Chinese Room}. An influential paper in software engineering research, Parnas and Clement's \citeyear{parnas1986rational} \textit{A rational design process: how and why to fake it}, explicitly recognise the value of fictions. Parnas and Clements write:

\begin{displayquote}
    ``We will never find a process that allows us to design software in a perfectly rational way. The good news is that we can \textit{fake it}. We can \emph{present} our system to others as \emph{if we} had been rational designers and it pays to \textit{pretend} [to] do so during development and maintenance. (\citeA{parnas1986rational}, p. 251; emphasis added). 
\end{displayquote}

Parnas and Clements explain the scope of the pretence and argue for its value in certain circumstances.

Finally, abstraction is fundamentally a pretence, for it presents a decontextualised and therefore simplified version of reality. Box \citeyear{box1997statistical} writes, ``\dots all models are wrong but some models are useful.'' We remove (neglect) details of a situation so as to frame that situation as a computational problem in order to provide a \textit{useful} (computational) solution to the problem. The question arises as to who is doing the framing, e.g., the stakeholders or the solution-providers.
% Jackson~\cite{jackson1995software} presents his \textit{Principle of the Dispassionate Methodologist}: ``The best advice comes from people who care more about your problem than about their solution.'' (\cite{jackson1995software}, p. 115)

% \section{Back to the story}

As Worley~\cite{Worley2014} recognises, a key element of storytelling is not only what is written (or said) but what the reader creates. One explanation for why the six-word story is effective is because the story creates `space' in the story for the reader to `complete' the story; in other words, the story creates `space' for multiple interpretations by the reader. As a reader we might, similar to Worley's wife, interpret the story as a tragedy concerning a mother and her baby. Or we might, as Worley says his wife's friend did, interpret the story as about someone who buys things for others but those things are not wanted. (If the reader wants an example of more direct experience to them, they might reflect on how reviewers' of their manuscripts or their grant applications seem to sometimes adopt wildly unexpected interpretations of what the reader wrote.)
% We might then, for example, imagine these six words as the seeds of a comedy about an uncle who always buys the wrong things.
These contrasting interpretations create different stories, despite the fact that the words of the story have not changed. Similarly, the \textit{same} reader might choose to interpret the story in different ways and draw contrasting meanings from the story, each time they re-read the story. One of the attractions of a reading group is that the participants bring different interpretations, and different experiences, of the story read, to share with the group.

\subsection{Representation}

It is clear that the six words of text, as a representation, requires interpretation; also that the models in the two figures, themselves representations, each require interpretation. One way we support interpretation is through additional words or notation, e.g., the notation used in Figure~\ref{subfigure:for-sale-object-diagram} and Figure~\ref{figure:advert} `tells' the reader, who has the appropriate knowledge, to interpret the representations in the figures as UML object diagrams. The captions to the figures obviously help with interpretation.

For software engineering, representations are unavoidable for they are essential to computational thinking. Representations are also problematic for software engineering because they allow -- even encourage -- \textit{multiple} interpretations of a representation \textit{and also}, therefore, allow for invalid interpretations. A common interpretation is necessary when more than one person is involved in the design, implementation, deployment and maintenance of a software system. For these kinds of reason, software engineers develop notations, specifications, protocols etc. 

For creative writers, such as Hemingway, representations are also essential, for they are the medium through which the writer's creations are communicated. Representations are an opportunity \textit{because} they allow -- even encourage -- \textit{multiple} interpretations of a representation and also, therefore, allow multiple \textit{valid} interpretations.

\subsection{Meaning}

The standards for validity -- for truth -- obviously differ between software engineering and creative writing.  What constitutes \textit{meaning} also differs. In computational thinking, the word ``meaning''  refers to the formalised semantics of a system. In Figure~\ref{figure:advert}, the statement, \texttt{anAdvert:Advert} \textit{means} that there is a a computational structure, i.e., an \texttt{object} with the identifier \texttt{anAdvert} that is an instance of the class, \texttt{Advert}. It also implies that there are likely several formal, computational operations we can do on the computational structure, such as invoke methods that are inherited from the class. 

In story-thinking, the word ``meaning'' is much harder to define. It concerns our individual relationship with ourselves and with the world, with what is important to us, with what resonates for us. In a way, this kind of meaning is best demonstrated through the telling of stories and the readers paying attention to how they respond and react to the story.

None of the formalised semantics is inherent within the figure, just as the meaning of the six-word story to Worley's wife is not inherent within the text. The information conveyed by the figure both suggests and constrains the ways we can think about the things represented by that figure. Similarly, the information conveyed by the six-word story both suggests and constrains the ways we can think about the things represented by that story. 

\subsection{Time}

Two distinctive aspects of the six-word story are that it represents things -- characters, events -- \textit{over time} and that these things are organised in a way that at least implies, if not makes explicit, some kind of causal relationship between them. For example, the shoes are for sale \textit{because} of some implied \textit{prior event}. The reader is left to wonder what the prior event was and how it is causing the sale of the shoes, e.g., the loss of a child, the purchase of unwanted clothing. In this particular story, and as an indication of the power of this story, the prior event that the reader `chooses' -- the prior event that the story `allows' the reader to choose through the `space' it provides to the reader -- brings meaning to the story \textit{for each reader}. By contrast, with our computational models, each model is intended to convey the same `objective' meaning for all readers.

There is a subtle cognitive effect taking place with a story, an effect that is not easily apparent with the six-word story we are discussing. Not only do the events of the story take place over the \textit{story's} time, but the \textit{reading} of the story, by the reader, itself takes place over time. The story's text is static, yet the reader \textit{experiences} an unfolding of events and actions and, perhaps most significantly, vicariously experiences the unfolding of the character or characters' experiences. With a UML object diagram, such as those given in Figure~\ref{subfigure:for-sale-object-diagram} and Figure~\ref{figure:advert}, there is no sense of an unfolding of the object. The model is static and, in a way, the experience of the model is static too. We might, over time, and through careful analysis of the model, gain more information from the model, but we don't experience a changing in the state of the thing being represented by the model.

UML object diagrams are not intended to represent temporal aspects of an object, class or system. We might instead turn to a state transition diagram, or a UML sequence diagram. Again, we might step our way though these diagrams, moving carefully from state to state. But again, the whole `lifetime' of the states is presented statically.

In a story, we can distinguish between the order in which events occurred in the story's world, and the order in which the events are told to the reader. In creative fiction, the author choose both sequences of events. In a memoir, the order in which events occurred in the memoirist's life are determined, but the memoirist may choose the order in which they recount those events. The memoirist can therefore control the order in which the events are presented.

\subsection{Particularity}

Another distinctive aspect of the six-word story is the representation of particulars \textit{as `first-class citizens'} of the story. Each thing in the story, each character, each event, is unique and is not an instance of a class of thing. In the story, the baby and the shoes are not instances of the class \texttt{baby} or the class \texttt{shoe}. By contrast, in Figure~\ref{subfigure:for-sale-object-diagram} and Figure~\ref{figure:advert}, each object is an instance of a class. Yet even though the story refers only to the particular, it allows for a universality. For example, where the reader interprets the story as about the tragedy of losing a child, the reader also gains an insight into the tragedy of losing each child. This is a different kind of thinking to losing an instance of the class child.

LaPlante~\cite{laplante2007making} writes: 
\begin{displayquote}
    It’s the opposite of abstraction, what we’re talking about here [i.e., writing short stories]. To abstract something is to dissociate something from a particular object. In other words, you move away from the very particular scene of a mother interacting with her truculent daughter and extrapolate `mother love.' That’s the reverse of what we do in writing [short stories]; we are talking about the act\dots [of associating]\dots a complex meaning with those most mundane of all things: sensory objects, people, and events.'' (\cite{laplante2007making}, p. 509). 
\end{displayquote}

\subsection{Point of view}

There is another distinctive element of stories that is not obviously present in the six-word: point of view. The story is not written in the first person, second person, or third person. In software engineering we often adopt the third person, e.g., the object diagrams. 

==> x_Old_material.tex <==
\section{Formatting instructions}

\subsection{Page size}

The paper should be A4 (21 $\times$ 29.7 cm or 8.27 $\times$ 11.69 inches). The margins around the text should be of 1 inch (2.54 cm) each and the text should be justified, not left-aligned/ragged. The length of the paper should not exceed the maximum 12 page limit. Pages should not be numbered.

\subsection{Fonts}

The fonts used in this paper are Times Roman or Times New Roman, Arial or Helvetica for headings and Courier for source code. Table~\ref{tbl:font-guide} summarises the font sizes and styles used for each part of this file. For Microsoft Word users, the default styles have been replaced to follow the settings here. For \LaTeX{} users, the \texttt{ppig.cls} applies the settings described here to your \texttt{.tex} file.

\begin{table}[h]
	\begin{center}
		\begin{tabular}{@{}cccc@{}}\toprule
			Type of text & Font & Font size & Style\\\midrule
			Paper title & Arial/Helvetica & 12pt & Bold\\
			Author names & Times Roman & 11pt & Bold\\
			Author affiliations & Times Roman & 11pt &\\
			The word "abstract" & Arial/Helvetica & 11pt & Bold\\
			Abstract text & Times Roman & 11pt &\\
			Section level 1 & Arial/Helvetica & 11pt & Bold\\
			Section level 2 & Arial/Helvetica & 11pt &\\
			Document text & Times Roman & 11pt & \\
			Caption & Times Roman & 11pt & Italic\\
			Code & Courier & 11pt &\\
			Bibliography & Times Roman & 11pt &\\
			Footnotes & Times Roman & 10pt &\\
			\bottomrule
		\end{tabular}
		\caption{Font guide.}
		\label{tbl:font-guide}
	\end{center}
\end{table}


\subsection{Title and authors}

The title, author's name(s) and affiliation(s) should be centred at the top of the first page. The title should be in Arial or Helvetica 12pt bold font. The author's name(s) should be in Times New Roman or Times Roman 11pt bold font, and their affiliation(s) should be in Times New Roman or Times Roman 11pt font.

The author's name(s) and affiliation(s) is created using a table with invisible borders and one row in Microsoft Word and a table with no borders and a row for each line in \LaTeX. In order to add a new author in Microsoft Word, add a new column to the table and enter the author's details. For \LaTeX users, please follow the instructions in the \texttt{ppig-submission-template.tex} file.

If all authors have the same affiliation, you may choose to have a single affiliation block, with author's name(s) and email address(es) separated by commas. To do so, use a single column table.

\subsection{References}

The references section at the end of this template shows the style that should be used for references. The references themselves should preferably follow the format of the APA (American Psychological Association) style guide, although we won't be too strict about the details. Citations should be in APA format: \citeA{blackwell1999how} says the year should be in parentheses after mention of the author's name. In cases where the author's name is not in the sentence, the citation gives name and year in parentheses \cite{blackwell1999how}.

\subsection{Figures and Tables}

Tables and Figures should fit within the boundaries of the text on this template file, and should be centred on the page. Both figures and tables can be placed inline with the text (e.g. Fig.~\ref{fig:sample-figure}), but the text shouldn't wrap around their sides. Use your own judgement to create suitable tables and figures. Figures and tables should have captions. Captions for both figures and tables should use the caption style defined in Table~\ref{tbl:font-guide}.

\begin{figure}[h]
	\centering
	\epsfig{file=sample-figure.eps, scale=0.5}
	\caption{A sample figure, with caption}
	\label{fig:sample-figure}
\end{figure}

\section{Submission Procedure}

Submissions must be in PDF format.

TBD
